Dilation two embedding one-by-one particular sub-quadtree into M-dimentional crossed cubes

In the parallel processing field, graph embedding is motivated by simulation interconnection networks to another. The quadtree is an important technique used to present spatial data and is used in many application domains, especially computer vision and image processing. Researchers are interested in the construction and manipulation of quadtrees on parallel machines. The crossed cubes consider an alternative to the ordinary hypercube. It offers many attractive properties. Significantly, it reduces diameter by a factor of 2 that of the ordinary cubes. Moreover, the crossed cubes have a great capacity to simulate other architectures. This paper is interested in the one-by-one dilation two embedding of a particular sub-quadtree graph into m-dimensional crossed cubes.

==> figures/actions.tex <==
\begin{table*}[h]
\centering
\setlength{\tabcolsep}{0.45\tabcolsep}
\begin{tabular}{|c|l|l|l|l|l|}
\hline
\multirow{12}{*}{\emph{f}}  & F1  & F2  & F3  & F4  & F5  \\ \cline{2-6} 
                         &  \emph{CPref$_{1}$00 := Asuff$_{1}$}    &  \emph{CPref$_{1}$01 := Asuff$_{1}$}    & \emph{CPref$_{1}$10 := Asuff$_{1}$}     & \emph{CPref$_{1}$11 := Asuff$_{1}$}     &  \emph{CPref$_{1}$01 := Asuff$_{1}$}    \\ \cline{2-6} 
                              & \emph{CPref$_{2}$00 := Asuff$_{2}$}    &  \emph{CPref$_{2}$00 := Asuff$_{2}$}   &  \emph{CPref$_{2}$10 := Asuff$_{2}$}   &   \emph{CPref$_{2}$11 := Asuff$_{2}$}  & \emph{CPref$_{2}$01 := Asuff$_{2}$}    \\ \cline{2-6} 
                              & \emph{CPref$_{3}$00 := Asuff$_{3}$}    & \emph{CPref$_{3}$00 := Asuff$_{3}$}    & \emph{CPref$_{3}$10 := Asuff$_{3}$}    & \emph{CPref$_{3}$01 := Asuff$_{3}$}    & \emph{CPref$_{3}$11 := Asuff$_{3}$}    \\ \cline{2-6} 
                              & F6  & F7  & F8  & F9  & F10 \\ \cline{2-6} 
                              & \emph{Cb$_{k}\bar{b}_{k+1}b_{k+2}\bar{b}_{k+3}$...00 := Asuff$_{1}$}   & \emph{Cb$_{k}\bar{b}_{k+1}\bar{b}_{k+2}$...00 := Asuff$_{1}$}  & \emph{CPref$_{j}$01 := Asuff$_{1}$}    &  \emph{CPref$_{j}$11 := Asuff$_{1}$}   &  \emph{CPref$_{j}$01 := Asuff$_{1}$}   \\ \cline{2-6} 
                              & \emph{CPref$_{2}$00 := Asuff$_{2}$}   &  \emph{CPref$_{2}$00 := Asuff$_{2}$}   & \emph{CPref$_{j}$10 := Asuff$_{2}$}     &  \emph{CPref$_{j}$00 := Asuff$_{2}$}   &  \emph{CPref$_{j}$10 := Asuff$_{2}$}   \\ \cline{2-6} 
                              &  \emph{CPref$_{3}$00 := Asuff$_{3}$}   &  \emph{CPref$_{3}$00 := Asuff$_{3}$}     &   \emph{CPref$_{j}$11 := Asuff$_{3}$}   &  \emph{CPref$_{j}$10 := Asuff$_{3}$}   &  \emph{CPref$_{j}$00 := Asuff$_{3}$}   \\ \cline{2-6} 
                              & F11 & F12 & F13 &     &     \\ \cline{2-6} 
                              &  \emph{CPref$_{j}$11 := Asuff$_{1}$}   &  \emph{CPref$_{1}$11 := Asuff$_{1}$}   &  \emph{CPref$_{1}$01 := Asuff$_{1}$}  &     &     \\ \cline{2-6} 
                              &  \emph{CPref$_{j}$00 := Asuff$_{2}$}   & \emph{CPref$_{2}$01 := Asuff$_{2}$}    &  \emph{CPref$_{2}$11 := Asuff$_{2}$}   &     &     \\ \cline{2-6} 
                              &  \emph{CPref$_{j}$01 := Asuff$_{3}$}   &  \emph{CPref$_{3}$11 := Asuff$_{3}$}   & \emph{CPref$_{3}$01 :=  Asuff$_{3}$}  &     &     \\ \hline
\multirow{16}{*}{\emph{f}$_{1}$} & F14 & F15 & F16 & F17 & F18 \\ \cline{2-6} 
                              & \emph{C0Pref$_{1}$00:=Asuff$_{1}$}    & \emph{C$\bar{0}$Pref$_{1-1}$01:=Asuff$_{1}$}    &  \emph{C$\bar{0}$Pref$_{1}$00:=Asuff$_{1}$}   &  \emph{C$\bar{0}$Pref$_{1-1}$11:=Asuff$_{1}$}   &  \emph{C$\bar{0}$b$_{k}b_{k+1}b_{k+2}\bar{b}_{k+3}$...00 := Asuff$_{1}$}    \\ \cline{2-6} 
                              &  \emph{C1Pref$_{1}$00:=Asuff$_{2}$}   &  \emph{C$\bar{1}$Pref$_{1-1}$01:=Asuff$_{2}$}    &  \emph{C$\bar{1}$Pref$_{1}$00:=Asuff$_{2}$}    &   \emph{C$\bar{1}$Pref$_{1-1}$01:=Asuff$_{2}$}  & \emph{C$\bar{1}$b$_{k}b_{k+1}b_{k+2}\bar{b}_{k+3}$...00 := Asuff$_{3}$}    \\ \cline{2-6} 
                              &  \emph{C1Pref$_{0}$00:=Asuff$_{3}$}   &  \emph{C$1$Pref$_{0}$10:=Asuff$_{3}$}   &  \emph{C$1$Pref$_{0}$01:=Asuff$_{3}$}   &   \emph{C$1$Pref$_{0}$10:=Asuff$_{3}$}  & \emph{C$1$Pref$_{0}$10:=Asuff$_{3}$}    \\ \cline{2-6} 
                              & F19 & F20 & F21 & F22 & F23 \\ \cline{2-6} 
                              &  \emph{C$\bar{0}$Pref$_{1}$11:=Asuff$_{1}$}   &  \emph{C$\bar{0}$Pref$_{j}$11:=Asuff$_{1}$}   & \emph{C$0$Pref$_{1}$01:=Asuff$_{1}$}    & \emph{C$0$Pref$_{1}$11:=Asuff$_{1}$}     &  \emph{C$\bar{0}$Pref$_{1-1}$11:=Asuff$_{1}$}   \\ \cline{2-6} 
                              &  \emph{C$\bar{1}$Pref$_{1}$10:=Asuff$_{2}$}   &  \emph{C$1$Pref$_{j}$01:=Asuff$_{2}$}   &  \emph{C$1$Pref$_{1}$11:=Asuff$_{2}$}   & \emph{C$1$Pref$_{1}$01:=Asuff$_{2}$}    &   \emph{C$\bar{1}$Pref$_{1-1}$01:=Asuff$_{2}$}  \\ \cline{2-6} 
                              & \emph{C$\bar{1}$Pref$_{0+1}$11:=Asuff$_{3}$}    &   \emph{C$\bar{1}$Pref$_{j}$10:=Asuff$_{3}$}  &  \emph{C$1$Pref$_{0}$01:=Asuff$_{3}$}    &  \emph{C$1$Pref$_{0}$11:=Asuff$_{3}$}   &  \emph{C$1$Pref$_{0}$00:=Asuff$_{3}$}   \\ \cline{2-6} 
                              & F24 & F25 & F26 & F27 & F28 \\ \cline{2-6} 
                              &  \emph{C$\bar{0}$Pref$_{1-1}$01:=Asuff$_{1}$}    &  \emph{C$\bar{0}$Pref$_{1}$10:=Asuff$_{1}$}   &  \emph{C$\bar{0}$Pref$_{1}$00:=Asuff$_{1}$}   &  \emph{C$\bar{0}$Pref$_{j}$01:=Asuff$_{1}$}   &  \emph{C$\bar{0}$Pref$_{j}$11:=Asuff$_{1}$}   \\ \cline{2-6} 
                              & \emph{C$\bar{1}$Pref$_{1-1}$01:=Asuff$_{2}$}    &  \emph{C$\bar{1}$Pref$_{1}$00:=Asuff$_{2}$}   &   \emph{C$\bar{1}$Pref$_{1}$10:=Asuff$_{2}$}  &  \emph{C$\bar{1}$Pref$_{j}$00:=Asuff$_{2}$}   &  \emph{C$\bar{1}$Pref$_{j}$10:=Asuff$_{2}$}   \\ \cline{2-6} 
                              & \emph{C$1$Pref$_{0}$10:=Asuff$_{3}$}  & \emph{C$\bar{1}$Pref$_{0+1}$10:=Asuff$_{3}$}     &  \emph{C$\bar{1}$Pref$_{0+1}$00:=Asuff$_{3}$}   &  \emph{C$\bar{1}$Pref$_{j}$00:=Asuff$_{3}$}   &  \emph{C$\bar{1}$Pref$_{j}$10:=Asuff$_{3}$}   \\ \cline{2-6} 
                              & F29 & F30 &     &     &     \\ \cline{2-6} 
                              & \emph{C$\bar{0}$Pref$_{j}$10:=Asuff$_{1}$}    &  \emph{C$\bar{0}$Pref$_{j}$00:=Asuff$_{1}$}    &     &     &     \\ \cline{2-6} 
                              & \emph{C$1$Pref$_{j}$11:=Asuff$_{2}$}    &  \emph{C$1$Pref$_{j}$01:=Asuff$_{2}$}   &     &     &     \\ \cline{2-6} 
                              &  \emph{C$\bar{1}$Pref$_{j}$00:=Asuff$_{3}$}   &  \emph{C$\bar{1}$Pref$_{j}$10:=Asuff$_{3}$}    &     &     &     \\ \hline
\end{tabular}
\caption{ffg zrg z gz rg zrg z rg zr gz rg z rg z rg zr gz rg z rg}
\end{table*}

$B \in E $ such that: $B=Cb_{k}b_{k+1}\dots b_{m-4}b_{m-3}b_{m-2}b_{m-1}$ = \emph{Cpref}$_{j}$$X_{1}X_{2}X_{3}X_{4}$ = \emph{Cpref}$_{j}$$X_{1}X_{2}adrr$  where $C={b_{0}, \bar{b}_{0}, \phi}$; adrr is the last 2 characters from a string B; \emph{pref}$_{j}$ = $b_{k}\dots b_{m-5}$ / $j=0 \hspace{0.25cm} if \hspace{0.25cm} b_{k}b_{k+1}=00 \hspace{0.25cm}; \hspace{0.25cm} j = 1 \hspace{0.25cm}  if \hspace{0.25cm} b_{k}\bar{b}_{k+1} \hspace{0.25cm};\hspace{0.25cm}  j=2  \hspace{0.25cm}  if \hspace{0.25cm}  \bar{b}_{k}b_{k+1} \hspace{0.25cm};\hspace{0.25cm}j=3  \hspace{0.25cm}  if \hspace{0.25cm} \bar{b}_{k} \bar{b}_{k+1}$. The number of super nodes \emph{CQ}$_{4}$ is equal to 2$^{m-4}$.\\ 

==> figures/case1.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l l}

\item 	\emph{f$_{1}$(0Pref$_{1}$00$X_{3}X_{4}$) := Asuff$_{1}$}& \\
\item 	\emph{f$_{1}$(1Pref$_{1}$00$X_{3}X_{4}$) := Asuff$_{2}$}&\\
\item   \emph{f$_{1}$(1Pref$_{0}$00$X_{3}X_{4}$) := Asuff$_{3}$}&\\
 OR & \\

\item 	\emph{f$_{1}$($\bar{0}$Pref$_{1}$00$X_{3}X_{4}$) := Asuff$_{1}$}&\\
\item 	\emph{f$_{1}$($\bar{1}$Pref$_{1}$00$X_{3}X_{4}$) := Asuff$_{2}$}& \\
\item   \emph{f$_{1}$(1Pref$_{0}$00$X_{3}X_{4}$) := Asuff$_{3}$}&\\
\end{tabular}
}
\end{table}


==> figures/case3.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l l l}
 •\emph{f$_{1}$($\bar{0}$Pref$_{1}$00$X_{3}X_{4}$) := Asuff$_{1}$}  & & •\emph{f$_{1}$($\bar{0}$Pref$_{1+(j-1)}$00$X_{3}X_{4}$) := Asuff$_{1}$}  \\
 •\emph{f$_{1}$($\bar{1}$Pref$_{1}$00$X_{3}X_{4}$) := Asuff$_{2}$}  & OR & •\emph{f$_{1}$(1Pref$_{1+(j-1)}$00$X_{3}X_{4}$) := Asuff$_{2}$}  \\
 •\emph{f$_{1}$($\bar{1}$Pref$_{0+1}$00$X_{3}X_{4}$) := Asuff$_{3}$}   & & •\emph{f$_{1}$($\bar{1}$Pref$_{0+j}$00$X_{3}X_{4}$) := Asuff$_{3}$}  \\
\end{tabular}
}
\end{table}

\begin{itemize}
\item 	\emph{f$_{1}$($\bar{0}$Pref$_{1}$00$X_{3}X_{4}$) := Asuff$_{1}$}
\item 	\emph{f$_{1}$($\bar{1}$Pref$_{1}$00$X_{3}X_{4}$) := Asuff$_{2}$}
\item   \emph{f$_{1}$($\bar{1}$Pref$_{0+1}$00$X_{3}X_{4}$) := Asuff$_{3}$} 
\end{itemize}
\vspace{-0.5cm}
\hspace{2,2cm} OR
\vspace{-0.5cm}
\begin{itemize}
\item 	\emph{f$_{1}$($\bar{0}$Pref$_{1+(j-1)}$00$X_{3}X_{4}$) := Asuff$_{1}$}
\item 	\emph{f$_{1}$(1Pref$_{1+(j-1)}$00$X_{3}X_{4}$) := Asuff$_{2}$} 
\item   \emph{f$_{1}$($\bar{1}$Pref$_{0+j}$00$X_{3}X_{4}$) := Asuff$_{3}$}
\end{itemize}

==> figures/edgen2.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{0}-\emph{01}  & \emph{00}-\emph{01}  \\ \hline
\emph{0}-\emph{02} &\emph{00}-\emph{10} \\ \hline
 \emph{0}-\emph{03}   & \emph{00}-\emph{10}-\emph{11}  \\ \hline
\end{tabular}
}
\caption{nodes embedding of \emph{PPQT}$_{2}$ into \emph{CQ}$_{2}$}
\end{table}


==> figures/edgen3.tex <==
\begin{table}[H]
\centering
\caption{edges embedding of \emph{PPQT}$_{3}$ into \emph{CQ}$_{4}$}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{0}-\emph{01}  & \emph{0000}-\emph{0100}  \\ \hline
\emph{0}-\emph{02} &\emph{0000}-\emph{1000} \\ \hline
 \emph{0}-\emph{03}   & \emph{0000}-\emph{1000}-\emph{1100}  \\ \hline
\end{tabular}
}

\end{table}


==> figures/edgen4.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{0}-\emph{01}  & \emph{000000}-\emph{010000}  \\ \hline
\emph{0}-\emph{02} &\emph{000000}-\emph{100000} \\ \hline
 \emph{0}-\emph{03}   & \emph{000000}-\emph{100000}-\emph{110000}  \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{4}$ into \emph{CQ}$_{6}$}
\end{table}


==> figures/edgen51.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{0}-\emph{01}  & \emph{0000000}-\emph{0010000}  \\ \hline
\emph{0}-\emph{02} &\emph{0000000}-\emph{0010000}-\emph{1010000} \\ \hline
 \emph{0}-\emph{03}   & \emph{0000000}-\emph{1000000}  \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{5}$ into \emph{CQ}$_{7}$ (situation 2,case 1}
\end{table}


==> figures/edgen52.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{03}-\emph{031}  & \emph{1000000}-\emph{1000001}  \\ \hline
\emph{03}-\emph{032} &\emph{1000000}-\emph{1000001}-\emph{0000011} \\ \hline
 \emph{03}-\emph{033}   & \emph{1000000}-\emph{1000010}  \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{5}$ into \emph{CQ}$_{7}$ (situation 2,case 2}
\end{table}


==> figures/edgen53.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{0331}-\emph{03311}  & \emph{1010010}-\emph{1010011}  \\ \hline
\emph{0331}-\emph{03312} &\emph{1010010}-\emph{0010010} \\ \hline
 \emph{0331}-\emph{03313}   & \emph{1010010}-\emph{0010010}-\emph{0010011}  \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{5}$ into \emph{CQ}$_{7}$ (situation 2,case 3}
\end{table}


==> figures/edgen54.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{01}-\emph{011}  & \emph{1010000}-\emph{1010001}  \\ \hline
\emph{01}-\emph{012} &\emph{1010000}-\emph{0110000}-\emph{0100000} \\ \hline
 \emph{01}-\emph{013}   & \emph{1010010}-\emph{0110000} \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{5}$ into \emph{CQ}$_{7}$ (situation 1,case 2}
\end{table}


==> figures/edgen81.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{0}-\emph{01}  & \emph{000000000000}-\emph{001000000000}  \\ \hline
\emph{0}-\emph{02} &\emph{000000000000}-\emph{001000000000}-\emph{101000000000} \\ \hline
 \emph{0}-\emph{03}   & \emph{000000000000}-\emph{100000000000}  \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{8}$ into \emph{CQ}$_{12}$ (situation 2,case 1}
\end{table}


==> figures/edgen82.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{03}-\emph{031}  & \emph{100000000000}-\emph{100010000000}  \\ \hline
\emph{03}-\emph{032} &\emph{100000000000}-\emph{100010000000}-\emph{000010000000} \\ \hline
 \emph{03}-\emph{033}   & \emph{100000000000}-\emph{100000000001}  \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{8}$ into \emph{CQ}$_{12}$ (situation 2,case 2}
\end{table}


==> figures/edgen83.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{01}-\emph{011}  & \emph{001000000000}-\emph{001010000000}  \\ \hline
\emph{01}-\emph{012} &\emph{001000000000}-\emph{011000000000}-\emph{110000000000} \\ \hline
 \emph{01}-\emph{013}   & \emph{001000000000}-\emph{111000000000}  \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{8}$ into \emph{CQ}$_{12}$ (situation 1,case 2}
\end{table}


==> figures/edgen84.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{011}-\emph{0111}  & \emph{001010000000}-\emph{001011000000}  \\ \hline
\emph{011}-\emph{0112} &\emph{001010000000}-\emph{001110000000}-\emph{001100000000} \\ \hline
 \emph{011}-\emph{0113}   & \emph{001010000000}-\emph{001110000000}  \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{8}$ into \emph{CQ}$_{12}$ (situation 1,case 2}
\end{table}


==> figures/edgen85.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\emph{PPQT} edge & crossed hypercube path \\ \hline
 \emph{0111}-\emph{01111}  & \emph{001011000000}-\emph{001011010000} \\ \hline
\emph{0111}-\emph{01112} &\emph{001011000000}-\emph{001011010000}-\emph{001010010000} \\ \hline
 \emph{0111}-\emph{01113}   & \emph{001011000000}-\emph{001011000001}  \\ \hline
\end{tabular}
}
\caption{edges embedding of \emph{PPQT}$_{8}$ into \emph{CQ}$_{12}$ (situation 2,case 1}
\end{table}


==> figures/tn53.tex <==
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
/   & / & \emph{03suff}$_{1}$ & \emph{1pref$_{0}$CQ}$_4$ \\ \hline
 /      &   /     & $03\textcolor{blue}{1}$     & 1$\textcolor{red}{00}0001$  \\ \hline
\emph{03suff}$_{2}$& \emph{0pref$_{0}$CQ}$_4$      & \emph{03suff}$_{3}$ &\emph{1pref$_{0}$CQ}$_4$ \\ \hline
$03\textcolor{blue}{2}$     & 1$\textcolor{red}{00}0001$       & $03\textcolor{blue}{3}$     & 1$\textcolor{red}{00}0010$  \\ \hline
\end{tabular}
}
\caption{level’s 3 nodes embedding of \emph{PPQT}$_{5}$ where \emph{suff}$_{p}=3$ into \emph{CQ}$_{7}$}
\end{table}


==> figures/tn68.tex <==
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
&\emph{Root}   & \emph{Prem(root)} & $0$\emph{suff}$_{1}$ & \emph{pref$_{1}$CQ}$_4$ \\ \hline
$\textcolor{blue}{0}$      & $\textcolor{red}{00}0000000$       & $0\textcolor{blue}{1}$     & $\textcolor{red}{01}0000000$  \\ \hline
$0$\emph{suff}$_{2}$& \emph{pref$_{2}$CQ}$_4$      & $0$\emph{suff}$_{3}$ & \emph{pref$_{3}$CQ}$_4$ \\ \hline
$0\textcolor{blue}{2}$     & $\textcolor{red}{10}0000000$       & $0\textcolor{blue}{3}$     & $\textcolor{red}{11}0000000$  \\ \hline
\end{tabular}
\begin{tabular}{|c|c|c|c|}
\hline
\emph{Root}   & \emph{Prem(root)} & $0$\emph{suff}$_{1}$ & $0$\emph{pref$_{1}$CQ}$_4$ \\ \hline
$\textcolor{blue}{0}$      & $0\textcolor{red}{00}000000000$       & $0\textcolor{blue}{1}$     & $0\textcolor{red}{01}000000000$  \\ \hline
$0$\emph{suff}$_{2}$& $1$\emph{pref$_{1}$CQ}$_4$      & $0$\emph{suff}$_{3}$ &$1$\emph{pref$_{0}$CQ}$_4$ \\ \hline
$0\textcolor{blue}{2}$     & $1\textcolor{red}{01}000000000$       & $0\textcolor{blue}{3}$     & $1\textcolor{red}{00}000000000$  \\ \hline
\end{tabular}
}
\caption{level’s 1, 2 nodes embedding of \emph{PQT}$_{6}$ into \emph{CQ}$_{9}$.}
\end{table}


==> reference.tex <==
\begin{thebibliography}{99}

\bibitem{c1} G. O. Young, ``Synthetic structure of industrial plastics (Book style with paper title and editor),'' 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15--64.
\bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123--135.
\bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
\bibitem{c4} B. Smith, ``An approach to graphs of linear forms (Unpublished work style),'' unpublished.
\bibitem{c5} E. H. Miller, ``A note on reflector arrays (Periodical styleÑAccepted for publication),'' IEEE Trans. Antennas Propagat., to be publised.
\bibitem{c6} J. Wang, ``Fundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),'' IEEE J. Quantum Electron., submitted for publication.
\bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
\bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),'' IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740--741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
\bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
\bibitem{c10} J. U. Duncombe, ``Infrared navigationÑPart I: An assessment of feasibility (Periodical style),'' IEEE Trans. Electron Devices, vol. ED-11, pp. 34--39, Jan. 1959.
\bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ``A clustering technique for digital communications channel equalization using radial basis function networks,'' IEEE Trans. Neural Networks, vol. 4, pp. 570--578, July 1993.
\bibitem{c12} R. W. Lucky, ``Automatic equalization for digital communication,'' Bell Syst. Tech. J., vol. 44, no. 4, pp. 547--588, Apr. 1965.
\bibitem{c13} S. P. Bingulac, ``On the compatibility of adaptive controllers (Published Conference Proceedings style),'' in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8--16.
\bibitem{c14} G. R. Faulhaber, ``Design of service systems with priority reservation,'' in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3--8.
\bibitem{c15} W. D. Doyle, ``Magnetization reversal in films with biaxial anisotropy,'' in 1987 Proc. INTERMAG Conf., pp. 2.2-1--2.2-6.
\bibitem{c16} G. W. Juette and L. E. Zeffanella, ``Radio noise currents n short sections on bundle conductors (Presented Conference Paper style),'' presented at the IEEE Summer power Meeting, Dallas, TX, June 22--27, 1990, Paper 90 SM 690-0 PWRS.
\bibitem{c17} J. G. Kreifeldt, ``An analysis of surface-detected EMG as an amplitude-modulated noise,'' presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
\bibitem{c18} J. Williams, ``Narrow-band analyzer (Thesis or Dissertation style),'' Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
\bibitem{c19} N. Kawasaki, ``Parametric study of thermal and chemical nonequilibrium nozzle flow,'' M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
\bibitem{c20} J. P. Wilkinson, ``Nonlinear resonant circuit devices (Patent style),'' U.S. Patent 3 624 12, July 16, 1990. 






\end{thebibliography}

